Streaming Video Model

Video understanding tasks have traditionally been modeled by two separate architectures, specially tailored for two distinct tasks. Sequence-based video tasks, such as action recognition, use a video backbone to directly extract spatiotemporal features, while frame-based video tasks, such as multiple object tracking (MOT), rely on single fixed-image backbone to extract spatial features. In contrast, we propose to unify video understanding tasks into one novel streaming video architecture, referred to as Streaming Vision Transformer (S-ViT). S-ViT first produces frame-level features with a memory-enabled temporally-aware spatial encoder to serve the frame-based video tasks. Then the frame features are input into a task-related temporal decoder to obtain spatiotemporal features for sequence-based tasks. The efficiency and efficacy of S-ViT is demonstrated by the state-of-the-art accuracy in the sequence-based action recognition task and the competitive advantage over conventional architecture in the frame-based MOT task. We believe that the concept of streaming video model and the implementation of S-ViT are solid steps towards a unified deep learning architecture for video understanding. Code will be available at https://github.com/yuzhms/Streaming-Video-Model.

==> sections/1_intro.tex <==



\section{Introduction}

% 1. Two types of video tasks: a. understand what is happening in a period of time, typical task: action recognition; b. identify key object or key information in a certain point of time in video; typical task: vod, mot, vos. We see discrepancy in handling these two types of tasks. 

% 2. The first type of video tasks usually adopt a clip-based video backbone, where research shows that spatial and temporal modeling should be interleaved. The second type of video tasks usually adopt an image backbone, without utilizing information from previous frames. Discuss their respective drawbacks. 

% 3. This is an effort to unify the two. We propose a unified backbone to serve both type of tasks. Describe the big picture: temporal aware spatial modeling + task-related temporal modeling. Differentiate with online video modeling or long-term video recognition. 

% 4. Describe our T2D-based architecture. How it works and its advantage. 

% 5. We used two downstream tasks, one from each category, to demonstrate the effectiveness of our proposal. Describe the two tasks and our results. 

% 6. Summarize our contributions: a. unified backbone for both types of video tasks; b. T2D-based implementation with high efficiency; c. achieved SOTA on two downstream tasks. 


Video is naturally a stream in our real world. Human watch a video and understand its content by seeing frames playing over time. Machines, on the country, are practically processing videos in a different manner. Most state-of-the-art video models require multiple frames to be fed as inputs at the same time and then process the entire video clip. Such block-processing models could only parse visual content in a short time period thus they have difficulty for real-world application where video is fed as an endless stream. For this reason, today's video model are usually applied for tasks that only involve short videos, and for more interesting tasks that cover steaming videos, image models are still in domination.


\begin{figure}[tb]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%   \includegraphics[width=0.95\linewidth]{figs/fig3.png}

   \caption{Comparison on video modeling paradigm on both streaming video tasks and clipped video tasks.}
   \label{fig:fig0}
\end{figure}

In this paper, we propose the idea of streaming video model to bridge the gap between video models and video tasks. The main obstruction for current video models to be used in streaming video \footnote{We use the term streaming video to refer videos with arbitrary length. The opposite is clipped videos with fixed and short length.} is its non-causal design. To be specific, in a typical video model like 3D convolution networks, the features for each video frame is not only related to features from previous frames but also related to features from future frames. That is to be said, the model has to see the entire video clip to compete the feature extraction. Intuitively, as human could understand the video without relying on futures, machines do not necessarily need future information to understand current frame as well. We thus have a change to remove the reliance on future frames in current video model without losing features' representative ability.

\begin{figure*}[th]
  \centering
%   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=0.95\linewidth]{figs/fig1.png}

   \caption{Illustration of streaming video model and classical clipped video model. (a) Clipped video model needs multiple frames as input and process them at the same time. (b) Streaming video model process videos frame by frame and transmit temporal information cross streaming video encoders.}
   \label{fig:fig1}
\end{figure*}

We therefore propose to build causal video model for streaming video processing. The central idea is removing the non-causal connection between the current frame and future frames, and then transferring the video processing pipeline to a frame-by-frame manner.
We implement this idea by building a novel \textit{streaming video model} called S-ViT (Streaming Vision Transformer) from a previous SOTA video model T2D-ViT. The key design in S-ViT is it uses cross attention to gather historical information from previous frames. When the model runs on a video stream, the feature of the first frame is extracted by self-attention inside the frame which is the same as an image model. S-ViT will additionally store the keys and values in attention as memory. When the second frame comes, beyond the inner-frame self-attention, the cross attention between the current frame and the stored memory is also calculated. Thanks to the triple 2D decomposition in T2D-ViT, the cross-attention is light-weight as only the correlation in the same horizontal and vertical directions are considered. Putting the inner-frame self-attention and cross-frame cross attention together, the proposed S-ViT model is able to model both static appearance information and dynamic motion information in an efficiency manner.

We select two types of tasks to evaluate the proposed S-ViT model. First is the traditional video task action recognition that operates on clipped videos. As our model produce image-level features instead of video-level features, we add an additional temporal aggregation model to extract a single video-level representation. The second is streaming video task that previously uses image models. Our streaming video model could directly replace the original image model as they both require a single image as input.

Our results demonstrate that S-ViT works well on both clipped video tasks and streaming video tasks. Specifically, on the Kinetics-400 action recognition dataset, we get the same performance compared to the baseline method T2D-ViT although we discard the attention calculation on future frames. On the MOT17 multiple object tracking dataset, S-ViT obtains significant performance gain over the image model counterpart and achieve competitive results when compared to state-of-the-art.

%S-ViT aims to process arbitrary number of frames in a streaming mode so that it is capable in both clipped video tasks and streaming video tasks. 
